High-speed quantum transducer with a single-photon emitter in a 2D resonator

Quantum transducers can transfer quantum information between different systems. Microwave-optical photon conversion is important for future quantum networks to interconnect remote superconducting quantum computers with optical fibers. Here we propose a high-speed quantum transducer based on a single-photon emitter in an atomically thin membrane resonator that can couple single microwave photons to single optical photons. The 2D resonator is a freestanding van der Waals heterostructure (may consist of hexagonal boron nitride, graphene, or other 2D materials) that hosts a quantum emitter. The mechanical vibration (phonon) of the 2D resonator interacts with optical photons by shifting the optical transition frequency of the single-photon emitter with strain or the Stark effect. The mechanical vibration couples to microwave photons by shifting the resonant frequency of a LC circuit that includes the membrane. Thanks to the small mass of the 2D resonator, both the single-photon optomechanical coupling strength and the electromechanical coupling strength can reach strong coupling regimes. This provides a way for high-speed quantum state transfer between a microwave photon, a phonon, and an optical photon.

==> README <==
+---------------------------------------------------------+
|            tabu - Flexible LaTeX tabulars               |
+---------------------------------------------------------+

tabu provides a single environment:          tabu
designed to make all kind of tabulars provided that they do
not split accross pages.

tabu is based on array.sty and requires no other package.
tabu does not modify array.sty nor the classes of tokens.

Starting from version 1.5, longtabu is provided: based on
longtable, longtabu allows tabulars to stretch out on
several pages.

tabu can be used in place of tabular, tabular* and tabularx
X columns in tabu can be specified with a width coefficient
the alignement (l,r,c,j) the column type (p,m,b) or even $.

tabu also works in math mode and its name remains tabu.
tabu can contain any type of tabular, array, tabularx
tabu can be put inside tabular, array, tabularx, tabular*

\begin{tabu} is like tabular if the preamble has no X column
\begin{tabu} to <dimen>      specifies the target width
\begin{tabu} spread <dimen>  enlarge the natural width

tabu with X columns has a default target if not specified
(usefull for nested tabus + compatibility with \linegoal)

tabu provides facilities to change the font and the alignment
in one row (\rowfont), save and restore the preamble and the
tabular parameters (\savetabu, \usetabu, \preamble).

tabu provides other facilities to align numbers in X columns
draw lines with color, dashed or even leaders. Those facilities
are provided for convenience: they work as long as the tabu
preamble does not contain "too special tokens".

tabu has been tested successfully with many packages related
to tabulars, cells, alignment...


